Learning to Sample: Counting with Complex Queries

We study the problem of efficiently estimating counts for queries involving complex filters, such as user-defined functions, or predicates involving self-joins and correlated subqueries. For such queries, traditional sampling techniques may not be applicable due to the complexity of the filter preventing sampling over joins, and sampling after the join may not be feasible due to the cost of computing the full join. The other natural approach of training and using an inexpensive classifier to estimate the count instead of the expensive predicate suffers from the difficulties in training a good classifier and giving meaningful confidence intervals. In this paper we propose a new method of learning to sample where we combine the best of both worlds by using sampling in two phases. First, we use samples to learn a probabilistic classifier, and then use the classifier to design a stratified sampling method to obtain the final estimates. We theoretically analyze algorithms for obtaining an optimal stratification, and compare our approach with a suite of natural alternatives like quantification learning, weighted and stratified sampling, and other techniques from the literature. We also provide extensive experiments in diverse use cases using multiple real and synthetic datasets to evaluate the quality, efficiency, and robustness of our approach.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=vldb

SAMPLES=paper.tex

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:	%.tex   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

paper.pdf: *.tex

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM) *.pdf *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'



==> bounds.tex <==
\section{Concentration Inequalities}

- unequal probability sampling without replacement can give lower variance and better estimates with lower samples but only if probabilities are proportional to size

- otherwise simple random sampling should be used

\subsection{Evaluating Performance of a Classifier}

- given a classifier on a limited sample of data, how can we make a judgement that our probabilities are proportional to size (with some error)?

- TBD: THIS WHOLE SECTION IS TBD!

\subsection{Concentration Inequalities of a Perfect Classifier}

- TBD: Can we use basic chernoff bounds, in other words, are classifier probabilities really independent? 

- Use the other method involving weighted sampling without replacement techniques (bound not based on independence) 

\subsection{A Looser Bound for a Non-Perfect Classifier}

Suppose our classifier is not perfect - some ratio of items may be mis-classifier as either 0 (from 1) or 1 (from 0), meaning that some probabilities are not ordered
according to the criteria needed in weighted sampling without probability. 

- TBD: formalize and solve the problem where our classifier is not always perfect. for a limited number of items, the classifier may produce probabilities that are
out of order (there may be some item with true label 0 that has higher probability than another item with true label of 1)

\subsection{Bounding the Sample Size}

- given our concentration inequalities, we can bound the number of samples

- the lower bound might be useful here from the Ratwani paper of O(sqrt(n)). 



==> challenges.tex <==






==> experiments.tex <==
\section{Experiments}\label{sec:expts}
\revc{In our experiments, we sought to understanding the following questions.
How well do the approaches work on real-world queries and data? When do the approaches fail?
How much does the performance of the classifier impact each approach?
What happens when the data is skewed or random? Can we tell when an approach is viable?
How do our approaches compare with existing work?}

We ran a series of experiments on real world datasets with a different query template defined for each dataset.
For each query, we changed the selectivity of the complex filter which controls the result size of the query.

\cutr{We used six different settings, ranging from XS \revm{to} XXL, where XS returns roughly 1\% of results, and XXL is roughly 90\% (see Figure~\ref{table:rss_queries}).

When comparing performance of each estimator, we commonly use interquartile range (IQR), which is defined as third quartile - first quartile. Interquartile range is
commonly used to measure the spread of a set of measurements and is less sensitive to outliers when describing the general spread of an estimator. 

The queries we have chosen are generic and can be executed in any number of data systems. Earlier, we have given SQL examples of two query templates (Listings~\ref{ex:k-skyband} and ~\ref{ex:k-distance}).}

\revc{Our experiments use three datasets and a variety of synthetic mixed datasets to analyze our approaches. We have previously defined SQL examples of two query templates (Listings~\ref{ex:k-skyband} and ~\ref{ex:k-distance}), and reuse the document analysis case study from \cite{lu_accelerating_2018}.
In addition, we evaluate performance on these queries when the data is mixed with synthetic data from different distributions, and the mixture rates are varied, providing a level of control over the randomness in the data.}
For our experiments, we implemented all approaches in Python 3. While there is a large difference in execution of queries across data systems, the user-defined function is still the primary time-bound and thus our comparisons should be valid regardless of data system.

Outside of the user defined function, we aimed to reuse core components to ensure efficiency, stability and robustness. Scikit-learn was used for classification methods: k-nearest neighbors (kNN), random forests (RF), and a simple two-layer neural network (NN). Pandas data analysis library was used for sampling, in particular weighted sampling without replacement. 

\begin{table*}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Dataset & XS & S & M & L & XL & XXL\\
\hline
Sports & 1\% (357) & 10\% (4841) & 29\% (13744) & 50\% (23589) & 70\% (32472) & 90\% (42432)\\
Neighbors & 2\% (1291) & 10\% (8568) & 25\% (17854) & 40\% (17854) & 75\% (55412) & 87\% (63341)\\
\hline
\end{tabular}
\caption{Result set sizes percent (exact) for real-world queries. Synthetic queries may be slightly different.}
\label{table:rss_queries}
\end{table*}


\subsection{Query Overview}
\paragraph{Type 1 - \textit{Sports}} This dataset contains information describing yearly statistics for players
in Major League Baseball. We use a selection of data describing pitching statistics, which excludes a portion of players (tuples).
It has about 47000 tuples, each describing a players performance by year.  For this dataset, we reuse the query in Example~\ref{ex:k-skyband}.
\reva{$k$ is varied to increase of decrease result set size.}

\paragraph{Type 2 - \textit{Neighbors}}
We used data from KDD Cup 1999, where the goal was to learn a predictive model that could distinguish between legitimate and illegitimate
(intrusion attacks) connections to a machine. There are 4.9 million records in the dataset with 41 features per record and a
binary label (normal or attack). We used a small sample of the dataset to validate our algorithms, with 73,000 tuples.
We adapted the query slightly for our task: record $i$ should be returned if there are no more than $k$ other
records within a distance $d$. This lets us adapt the size of the result set for experimental validation of our algorithms. This query is
defined in the introduction, see Listing \ref{ex:k-distance}. $d$ is varied to increase or decrease result set size.

\paragraph{Type 3 - \textit{Text Categories}}
\reva{Query and dataset is the same as in \cite{lu_accelerating_2018}. Data is from the LSHTC \cite{partalas2015lshtc} text dataset, consisting of 2.4M documents from Wikipedia along with their categorization.
Query is to find the number of documents with greater than $c$ categories, and the result size is varied by changing $c$.}
\subsection{Notations}
We compared the following approaches throughout our experiments. Unless specifically mentioned, learning-based approaches using the same classifier setup: classifier type and parameters are kept constant, although they may learn
different models due to sampling.
\begin{table}[h]
  \centering
  \begin{tabular}{|l|l|}
    \hline
    Notation & Description\\
    \hline
    RS & Simple Random Sampling\\
    SS & Stratified Sampling (Proportional)\\
    QL & Quantification Learning\\
    QLCC & QL using Classify and Count\\
    QLAC & QL using Adjusted Count\\
    QLSC & QL with Sample Clean\\
    PPS & Probabilistic Predicates with Scaling\\
    LSS & Learned Stratified Sampling\\
    LWS & Learned Weighted Sampling\\
    \hline
  \end{tabular}
  \caption{Notations used for denoting approaches in experiments. \label{table:expr_notations}}
\end{table}
\subsection{Sampling Comparisons}
\reva{
\begin{figure*}[h]
  \centering
  \includegraphics[width=.9\linewidth]{figs/text_estimate_vs_method_ss_01_violin}
  \caption{\label{fig:text_estimate_query_method} Estimates on text query for different category parameters, resulting in varying result sizes.}
\end{figure*}

\begin{figure*}[ht]
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Neighbors}
    \includegraphics[width=.99\textwidth]{figs/E-distance-all-line-2pct-sample}
    \label{fig:lws-comparison-distance}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Sports}
    \includegraphics[width=.99\textwidth]{figs/E-kskyband-all-line-2pct-sample}
    \label{fig:lws-comparison}%
  \end{subfigure}
  \caption{Mean absolute error of sampling procedures for estimating counts. Result sizes are modified by changing query parameters. Total sample size is 2\%.}
  \label{fig:overall-sampling-lws}
\end{figure*}
}
\reva{We start our experiments with an in-depth discussion of the approaches on the text categories query in Figure~\ref{fig:text_estimate_query_method}. We use a 1\% sample (17k), which is a challenging scenario for classifiers on text data.
Result sizes tend to be skewed: documents with seven categories (Figure~\ref{fig:text_estimate_query_method} left) comprise under ~10\% of the data, where figures with at least two categories comprises a majority of the data.
This experiment highlights an important distinction of LSS from QL-based approaches: QL-based approaches depend much more heavily on the performance of the classifier then LSS does.

In situations where the dataset is skewed, the classifier predicts either 1 or 0 for most documents. Thus, QLCC, which uses no modifiers from the initial count, behaves quite poorly. Adjusting this count is the only difference between
QLCC and QLSC/QLAC.
As this adjustment is done by using estimated error metrics we analyzed the impact this had on final estimation quality  (Table~\ref{table:text_fpr_tpr}).
While the exact calculations are different for each estimation procedure, we used the differences of TPR and FPR between sample and actual values to gain insight.
Of utmost importance, for many category settings TPR=FPR, which is expected when a classifier is no better than random chance \cite{powers2011evaluation}.


Furthermore, estimated error rates are often quite different from actual TPR, FPR values, leading to situations where QLSC or QLAC over or under estimate by a significant margin.
This is particularly troublesome in skewed situations with a poor classifier (in other words, one of FPR or TPR is poor). In these settings, adjustments can produce high variance in estimates. }

\revb{We compared our approaches to existing work based on probabilistic predicates \cite{lu_accelerating_2018} (PPS).
This is a slightly modified version of their approach to work with counting queries where the second round of sampling is used to estimate the total by calculating the mean of the predictions and then computing the scaled estimate.
PPS has many of the same characteristics as QLCC, but also suffers from relying on the mean of the predicted labels. In our experiments, QLSC generally produces better estimates.
As this is similar to QLSC and other QL-based approaches, we leave PPS out for the rest of the comparisons.}

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
  \hline
 Result Size & \multicolumn{2}{c|}{Sample Rate} & \multicolumn{2}{c|}{Actual Rate}\\
  \hline
  & TPR & FPR & TPR & FPR\\
  \hline
  117k & 0 & 0 & .004 & 0\\
  246k & 0 & .006 & 001 & .002\\
  550k & .01 & .34 & .03 & .18\\
  857k & .35 & .95 & .53 & .85\\
  1.3M & .79 & .99 & .86 & .99\\
  \hline
\end{tabular}
\caption{Sample and Actual TPR and FPR values for text classifers. \label{table:text_fpr_tpr}}
\end{table}

\reva{We also examined datasets where classifier performance was better (Sports and Neighbors). Figure ~\ref{fig:overall-sampling-lws} shows mean absolute error (MAE) compare to result size as we varied parameters for each query.
The classifier model and parameters were kept constant across learning based methods.
F1 scores averaged .85 and .80 for ~\ref{fig:overall-sampling-lws}a and ~\ref{fig:overall-sampling-lws}b, respectively (with small sizes being more difficult).
QL-based methods are more competitive here, but LSS (highlighted) has consistenly lower MAE. There are a few cases where QLCC performs better due to the high accuracy and precision of the underlying classifier.
There are only two settings out of twelve where QLSC or QLAC has lower MAE than QLCC. Overall accuracy of the classifier itself, combined with differences in TPR/FPR between estimate and real mentioned above, imply classifier adjustments not necessary
when the classifier has a high F1-Score. However, referring back to Figure~\ref{fig:text_estimate_query_method}, QLSC performs quite well in comparison to QLAC and QLCC. QLSC appears to be the most robust of the QL-based approaches, but does not perform
as well as LSS.}

\subsection{LSS vs. LWS} \label{ssec:lssvslws}
We continue our experiments with a comparison of LWS and LSS with SS and \SRS (Figure ~\ref{fig:lss_vs_lws}). Both LSS and LWS used a random forest classifier (n=100 estimators) and a 25\% training:sampling split.
\SSP and LSS used 4 strata. SSwas based on the join/filter attributes (which resulted in 2-dimensional strata).
LSS and LWS generated estimate distributions with consistently smaller IQR's than SS and RS, although LWS is more susceptible to producing outliers.
\reva{Of particular note is that, while LWS is an unbiased estimator, the performance of the classifier influences whether or not results are typically below or above the expected value. When
the result size is XS (roughly 1\% of the data is included in the result), the classifier generates more false negatives and is more likely to produce an underestimate. In general, LWS estimation is affected more by false negatives/positives moreso
than LSS does. Overall, LSS is consistently the highest quality estimator.}


\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{figs/E-distance-lws}
  \caption{\label{fig:lss_vs_lws}Estimates vs. Method for Neighbors query at 2\% sample size.}
\end{figure}

\subsection{Runtime and Scalability}
Before we examine characteristics of individual methods, we provide a brief look into the performance of our approaches. Both LWS and QL are simpler than LSS, which has additional overhead in stratification. Thus, we only look at results from LSS.

\begin{figure}[h]
  \centering
  \includegraphics[width=.5\linewidth]{figs/runtime_by_category_kskyband}
  \caption{\label{fig:execution_time_overhead}Execution time overhead vs sample size (in thousands) for LSS, broken down by key phases.}
\end{figure}

In Figure~\ref{fig:execution_time_overhead}, we plot the overhead added by using LSS when compared to SS. There are three distinct overhead phases. P1 Learning represents the time to perform initial RS, following by machine learning training. P1 Sample Design includes variance estimates and strata layout algorithm. P2 Overhead includes time of classification and iteration, and sampling. We listed the percentage of total runtime used by our overhead (top of each bar). Note that these are miniscule: .20\%!

\subsection{Examining Characteristics of LSS}
We tested a variety of facets involved in LSS: how strata are laid out, the number of strata, sample allocation to each phase, and how the performance of the underlying classifier affects estimate quality. 

\subsubsection{Strata Layout Strategy}
In this experiment we tested various methods of strata layout (Figure~\ref{fig:lss:ssp:num_strata}). Each approach used 4 strata. In fixed width, the strata are laid out in even increments. Fixed height ensures each strata has an identical number of elements, and optimal width selects the strata boundaries by minimizing the variance of elements from the first phase of sampling.

It is no surprise that fixed height produces poor results for stratified sampling, as each strata may contain a mixture of labels. In particular, for skewed datasets where one label occurs more often(XS and XXL), fixed height has much higher variance in its estimate. The violin plots shows the effectiveness of our strata layout optimizations (Section~\ref{sec:approach:lss:stratify}). Specifically, using our optimizations, the interquartile range of LSS is much smaller than the naive, fixed-width approach. That is, the estimates vary less than the naive strategy.

\subsubsection{Number of Strata}
In this experiment (Figure~\ref{fig:lss:ssp:num_strata}), we investigate the effect of number of strata on estimation quality when using LSS. We also compared LSS to SS when both were given an identical number of strata.  We varied the number of strata with 4, 9, 25, 49, and 100 strata available. Sports (Figure~\ref{fig:kskyband-number-bins-ss}) is an ideal query for \SSP: all the results are in a few strata (especially in XS, S result sizes). Thus, it's expected that \SSP performs extremely well with a high number of strata.

\begin{figure*}[ht]
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Neighbors}
    \includegraphics[width=.99\textwidth]{figs/E-distance-bin-analysis-ss.png}
    \label{fig:distance-number-bins-ss}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Sports}
    \includegraphics[width=.99\textwidth]{figs/E-kskyband-bin-analysis-ss.png}
    \label{fig:kskyband-number-bins-ss}%
  \end{subfigure}
  \caption{Performance comparison of LSS and \SSP across varying buckets. Each row is a different sample size (1\%, 2\%), and each column represents a change of parameters resulting in a different result set size (XS, S, L).}
  \label{fig:lss:ssp:num_strata}
\end{figure*}

As expected, increasing strata improves estimation quality, but not substantially so. In the extreme case (XS), \SSP is very competitive whereas LSS produces an occasional outlier. However, the interquartile range of LSS is smaller than \SSP.  For both query types and all result sizes, interquartile range of LSS is  substantially smaller than SS. 

\subsubsection{Sample Split}

In this experiment (Figure~\ref{fig:sample_split} we tested the effects of sample allocation between phases: learning and sampling. We tested splits of 10, 25, 50, and 75 percent. A 10 percent split means that only 10\% of the sample size is used towards training a classifier, with the remainder being used to produce an estimate by learned stratified sampling.

Under 10\% samples, LSS tends to have a larger IQR than other proportions, and generates more extreme estimations. Conversely, overly large first phase allocations reduce the number of samples available to produce an estimate and can have a similar effect. Both middle proportions (25\% and 50\%) consistently produce the most reliable estimates with lowest IQR's, and minimal outliers. Number of strata was fixed at 4.

\begin{figure*}[ht]
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Neighbors}
    \includegraphics[width=.99\textwidth]{figs/E-distance-sample-split.png}
    \label{fig:distance-sample-split}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Sports}
    \includegraphics[width=.99\textwidth]{figs/E-kskyband-sample-split.png}
    \label{fig:kskyband-sample-split}%
  \end{subfigure}
  \caption{Performance comparison of LSS as the ratio of samples used in classifier training to sampling phases is changed. Each row is a different sample size (1\%, 2\%), and each column represents a change of parameters resulting in a different result set size (XS, S, L).}
  \label{fig:sample_split}
\end{figure*}

\subsubsection{Effect of Classifier Quality on LSS}

As LSS is driven by probabilities produced by a classifier, it is naturally dependent on the classifier itself. We tested LSS on four different classifiers (Figure~\ref{fig:classifiers}):  k-Nearest Neighbors (KNN), simple two-layer neural network (5, 2 intermediate layers) (NN),  random forest classifier (n=100 estimators), and a dummy classifier (Random) that generated arbitrary random probabilities. Random can be viewed as a worst case scenario for LSS as the desired effect of stratification (producing homogenous strata) is completely lost. Across classifiers, proportion of training:sampling was 25\%, and number of strata is 4.  

Consistent with the theory behind stratified sampling and optimal allocation, a classifier that performs better than random produces higher quality estimates. It also validates the approach: even if a classifier performs poorly (Random), our estimation procedure still produces estimates with a quality relative to traditional stratified sampling.

\begin{figure*}[ht]
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Neighbors}
    \includegraphics[width=.99\textwidth]{figs/E-distance-classifiers.png}
    \label{fig:distance-number-bins}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\textwidth}
    \caption{Sports}
    \includegraphics[width=.99\textwidth]{figs/E-kskyband-classifiers.png}
    \label{fig:kskyband-number-bins}%
  \end{subfigure}
  \caption{Performance comparison of LSS for different classifiers. Each row is a different sample size (1\%, 2\%), and each column represents a change of parameters resulting in a different result set size (XS, S, L).}
  \label{fig:classifiers}
\end{figure*}

\subsection{Synthetic Datasets}
\revc{We generated a set of "noisy" datasets where we controlled the level of noise added to the baseline Sports dataset. As each element in the query has a filter applied to it (in this case, \texttt{COUNT(*) <= k}), we added noise to \texttt{COUNT} for each element based on a mixture
parameter $\alpha$. Let $x$ be the original value, and $x'$ be the random value. We define the new value as $y = (1-\alpha)x + \alpha x'$. New values were generated from two distributions: standard normal and Zipfian.
Zipfian was used to index into a randomly permuted array of potential \texttt{COUNT} values compiled from the original values. Thus, as $alpha$ approaches 1, values are computed entirely using the distributions.

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{figs/mae_vs_alpha_kskyband_gaussian}
  \caption{\label{fig:synthetic_gaussian}MAE vs. Alpha for Sports dataset.}
\end{figure}

In Figure~\ref{fig:synthetic_gaussian}, we plotted MAE vs. $alpha$ for LSS, RS, and QLSC when values are mixed with a standard normal. Grey dashed line is the result size.
The original data is quite skewed: each element tends to have a quite low inner count value (that is, a high number of elements pass the initial filter, but the range is high).
Therefore, as $alpha$ increases the result size tends to decrease as each inner count is mixed with a (probably) higher value.
Until $alpha$ reaches $.5$, LSS and QLSC outperform RS with LSS being slightly better. At that point, the data tends to be less correlated and less predictable.

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{figs/mae_vs_zipf_kskyband_zipfian}
  \caption{\label{fig:synthetic_zipf}MAE vs. Zipf parameter for Sports dataset where mixing parameter $\alpha$ was fixed at .6. There were 100 runs per generated dataset (value of Zipf).}
\end{figure}

We also tested how drawing from skewed distributions effects the classifier. We varied the $s$ value in Zipfian distributions to induce randomness, but for each $s$ we kept the generated distribution fixed over 100 runs.
Thus, each $s$ value has a chance to generate a randomly skewed dataset (the original data is already quite skewed).
Figure~\ref{fig:synthetic_zipf} shows clearly how randomness impacts the performance of each approach.
Dotted line shows the F1 Score for each mixture distribution generated. Sampling induces slight variances in F1-Scores within distributions but are mostly consistent. Importantly, there is a clear correlation between performance of QLSC and LSS
and F1-Score. MAE is highest for both LSS and QLSC when the average F1-Score is lowest and RS is better. This intuitively makes sense: if the underlying classifier performs so poorly that it is worse than random choice, resulting estimations will also be poor.}

